Probabilistically Safe Robot Planning with Confidence-Based Human Predictions

In order to safely operate around humans, robots can employ predictive models of human motion. Unfortunately, these models cannot capture the full complexity of human behavior and necessarily introduce simplifying assumptions. As a result, predictions may degrade whenever the observed human behavior departs from the assumed structure, which can have negative implications for safety. In this paper, we observe that how "rational" human actions appear under a particular model can be viewed as an indicator of that model's ability to describe the human's current motion. By reasoning about this model confidence in a real-time Bayesian framework, we show that the robot can very quickly modulate its predictions to become more uncertain when the model performs poorly. Building on recent work in provably-safe trajectory planning, we leverage these confidence-aware human motion predictions to generate assured autonomous robot motion. Our new analysis combines worst-case tracking error guarantees for the physical robot with probabilistic time-varying human predictions, yielding a quantitative, probabilistic safety certificate. We demonstrate our approach with a quadcopter navigating around a human.

==> (RSS 2018) Quadcopters for the People/conclusion.tex <==
\vspace{-.1cm}
\section{Discussion \& Conclusion}
\label{sec:conclusion}
\vspace{-.1cm}
%\adnote{dont have discussion and conclusion, just discussion, and separate into summary and limitations+future work}
In this paper, we interpret the ``rationality'' coefficient in the human decision modeling literature as an indicator of the robot's confidence in its ability to predict human motion. We formulate this confidence $\beta$ as a hidden state that the robot can infer by contrasting observed human motion with its predictive model. %Marginalizing over this hidden state, the robot can quickly adapt its forecasts to effectively reflect the predictability of the human's motion in real time. %The resulting predictions of human motion are \textit{probabilistic} and \textit{time-varying}. 
Marginalizing over this hidden state, the robot can quickly adapt its forecasts to effectively reflect the predictability of the human's motion in real time. We build on the theoretical analysis of the provably safe FaSTrack motion planning scheme to construct a novel probabilistic safety certificate that combines worst-case and probabilistic analysis, and show that the resulting trajectories are collision-free at run-time with high probability. 

We compare our $\beta$ inference technique to two fixed-$\beta$ approaches, all using our proposed probabilistically safe motion planning scheme. Our results indicate that, even though the three methods perform similarly when the human's motion is well-explained by the robot's model, inferring $\beta$ yields safer and more efficient robot trajectories in environments with unmodeled obstacles or unmodeled human goals. %where the human moves to avoid unmodeled obstacles. %Our method also produces more efficient robot trajectories in environments with either unmodeled obstacles or unmodeled human goals. 
Future work should investigate more complex human motion, closed-loop interaction models, and navigating around multiple humans.

%\vspace{-.5cm}
%Although future work should investigate more complex human models that can improve the prediction confidence, even with a simple human motion model we can generate and track plans that do not compromise the safety or effectiveness of our robot.




%An interesting direction for future work will be to investigate the performance of our $\beta$ inference on coupled interactions between the human and robot. %method in more varied human-robot interactions, perhaps involving multiple humans and robots. Additionally, future inquiry might analyze the coupled interaction between human and robot induced by our method of inferring $\beta$. 

% FUCK FUTURE WORK
% Another promising direction is to reformulate the notion of probabilistic safety in Sec. \ref{sec:solution_plan} to be robust to errors in time-varying probability distributions generated by the human motion predictor. Finally, there is much work yet to do before the techniques presented here can scale to higher-dimensional human and robot state and action spaces, multi-human and multi-robot scenarios.% and real world interactions in crowded, chaotic environments.

%\dfknote{Will this technique lead to overly conservative robots?}

%\adnote{humans will adapt to the robot too (here we can cite unfreezing robot and dorsa and stefanos mutual adaptation); although we didn't account for that in this paper, the method for re-estimating beta still stands even if we model the person's reward on also depending on the robot's actions }

==> (RSS 2018) Quadcopters for the People/experiments.tex <==
\section{Demonstration with Real Human Trajectories}
\label{sec:demo}

We implemented real-time human motion prediction with $\beta$ inference and safe probabilistic motion planning via FaSTrack within the Robot Operating System (ROS) framework \cite{quigley2009ros}. To demonstrate the characteristic behavior of our approach, we created three different environment setups and collected a total of 48 human walking trajectories (walked by 16 different people). The trajectories are measured as $(x, y)$ positions on the ground plane at roughly 235 Hz by an OptiTrack infrared motion capture system.\footnote{We note that in a more realistic setting, we would need to utilize alternative methods for state estimation such as lidar measurements.} 
We also demonstrated our system in hardware on a Crazyflie 2.0 platform navigating around a person in a physical space.\footnote{\url{https://youtu.be/2ZRGxWknENg}}  

\textbf{Environments.} In the first environment there are no obstacles and the robot is aware of the human's goal. The second environment is identical to the first, except that the human must avoid a coffee spill that the robot is unaware of. In the third environment, the human walks in a triangular pattern from her start position to two known goals and back. 

%\textbf{Environments.} In the first environment there are no obstacles and the robot is aware of the human's goal. Here, the human's motion may be interpreted as rational \textit{with respect to the robot's model of the human.} The second environment is identical to the first, except that the human must avoid a coffee spill that the robot is unaware of. In this case, the human appears irrational due to the unmodeled obstacle. In the third environment, the human walks in a triangular pattern from her start position to two known obstacles and back. Her motion to each of the known goals appears rational to the robot, however her return to the start point appears irrational to the robot.

\textbf{Evaluated Methods.} For each human trajectory, we compare the performance of our adaptive $\beta$ inference method with two baselines using fixed $\beta \in \{0.05, 10\}$. When $\beta = 0.05$, the robot is unsure of its model of the human's motion. This low-confidence method cannot trust its own predictions about the human's future trajectory. On the other hand, the $\beta = 10$ high-confidence method remains confident in its predictions even when the human deviates from them. These two baselines exist at opposite ends of a spectrum. Comparing our adaptive inference method to these baselines provides useful intuition for the relative performance of all three methods in common failure modes (see Fig.~\ref{fig:coffee_three_quadrotor}).

\textbf{Metrics.} We measure the performance of our adaptive $\beta$ inference approach in both of these cases by simulating a quadcopter moving through the environment to a pre-specified goal position while replaying the recorded human trajectory. We simulate near-hover quadcopter dynamics with the FaSTrack optimal controller applied at 100 Hz. For each simulation, we record the minimum distance in the ground plane between the human and the quadcopter as a proxy for the overall safety of the system. The quadcopter's travel time serves to measure its overall efficiency.%We use the total time for the quadcopter to reach its goal in each simulation as a measure of its overall efficiency.

In each environment, we compute the safety metric for all 16 human trajectories when applying each of the three human motion prediction methods and display the corresponding box and whisker plots side by side. To compare the efficiency of our approach to the baselines we compute the difference between the trajectory completion time of our approach, $T_{\textnormal{infer}}$, and that of the low and high confidence baselines, $\{T_{\textnormal{lo}}, T_{\textnormal{hi}}\}$. If the resulting boxplots are below zero, then $\beta$ inference results in faster robot trajectories than the baselines on a per-human trajectory basis.\footnote{The upper and lower bounds of the box in each boxplot are the $75^{\text{th}}$ and $25^{\text{th}}$ percentiles. The horizontal red line is the median, and the notches show the bootstrapped $95\%$ confidence interval for the population mean.}

% \noindent\textbf{Hypothesis.}
% \adnote{ hypothesis: inferred captures the best of both worlds; note: i think people will wonder what about a fixed medium beta?}

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.95\textwidth]{coffee_nocoffee_2x2.jpg}
    \caption{Safety and efficiency metrics in a complete environment and one with an unmodeled obstacle.}
    \label{fig:coffee_nocoffee}
    \vspace{-.55cm}
\end{figure*}

\textbf{Complete Model.}
\label{subsec:complete_model} First, we designed an example environment where the robot's model is complete and the human motion appears to be rational. In this scenario, humans would walk in a straight line from their start location to their goal which was known by the robot \textit{a priori}. 

When the robot has high confidence in its model, the human's direct motion towards the goal appears highly rational and results in both safe (Fig.~\ref{fig:coffee_nocoffee}, top left) and efficient plans (Fig.~\ref{fig:coffee_nocoffee}, bottom left). We see a similar behavior for the robot that adapts its confidence: although initially the robot is uncertain about how well the human's motion matches its model, the direct behavior of the human leads to the robot to believe that it has high model confidence. Thus, the $\beta$ inference robot produces overall safe and efficient plans. Although we expect that the low-confidence model would lead to less efficient plans but comparably safe plans, we see that the low-confidence robot performs comparably in terms of both safety and efficiency. 

Ultimately, this example demonstrates that when the robot's model is rich enough to capture the environment and behavior of the human, inferring model confidence does not hinder the robot from producing safe and efficient plans.

\textbf{Unmodeled Obstacle.}
\label{subsec:unmodeled_obstacle} Often, robots do not have fully specified models of the environment. In this scenario, the human has the same start and goal as in the complete model case except that there is a coffee spill in her path. This coffee spill on the ground is unmodeled by the robot, making the human's motion appear less rational. 

When the human is navigating around the unmodeled coffee spill, the robot that continuously updates its model confidence and replans with the updated predictions almost always maintains a safe distance (Fig.~\ref{fig:coffee_nocoffee}, top right). In comparison, the fixed-$\beta$ models that have either high-confidence or low-confidence approach the human more closely. This increase in the minimum distance between the human and the robot during execution time indicates that continuous $\beta$ inference can lead to safer robot plans. 

For the efficiency metric, a robot that uses $\beta$ inference is able to get to the goal faster than a robot that assumes a high or a low confidence in its human model (Fig.~\ref{fig:coffee_nocoffee}, bottom right). This is particularly interesting as overall we see that enabling the robot to reason about its model confidence can lead to \textit{safer} and \textit{more efficient} plans. 
%\abnote{do we want to call out how inference does much better compared to the high-confidence model because it erroneously reasons about the behavior and is forced to re-plan more/further?} 

%When a robot observes human motion, unmodeled obstacles that force people to replan can make it difficult for the robot to understand and predict the human's motion. To analyze how different human model confidence measures affect the robot's plan in such a scenario, we compared a simple environment with no obstacles to an environment with an unmodeled coffee spill that is in the human's way. In this scenario, humans were instructed to walk to a single goal and the robot would attempt to navigate to its own goal while the human was walking in the same space. 


% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figs/safety_metric.pdf}
%     \caption{When the human deviates from the expected motion because of the unmodeled coffee spill, a robot is inferring $\beta$ online maintains a further distance from the human. In contrast, the fixed-$\beta$ methods get closer to the human, potentially compromising safety.}
%     \label{fig:safe_coffee_results}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figs/safety_metric_nocoffee.png}
%     \caption{When the robot's model fully describes the human's motion, all confidence measures perform comparably and lead to predictions and plans that stay away from the human.}
%     \label{fig:safe_nocoffee_results}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figs/efficiency_metric.pdf}
%     \caption{In this scenario, unmodeled coffee prevents the human from taking a predictable path to their goal. We show the difference between the total executed trajectory time of the $\beta$ inference method ($T_{\text{infer}}$) with the low ($T_{\text{lo}}$) and high ($T_{\text{hi}}$) confidence method. The robot that infers the model confidence is consistently faster than both the low and high confidence methods.}
%     \label{fig:eff_coffee_results}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figs/efficiency_metric_nocoffee.png}
%     \caption{As expected, when humans move rationally to their goal, the $\beta$ inference method produces similarly fast trajectories to the low and high confidence methods.}
%     \label{fig:eff_nocoffee_results}
% \end{figure}


\textbf{Unmodeled Goal.}
\label{subsec:unmodeled_goal} In most realistic human-robot encounters, even if the robot does have an accurate environment map and observes all obstacles, it is unlikely for it to be aware of all human goals. We test our approach's resilience to unknown human goals by constructing a scenario in which the human moves between both known and unknown goals. The human first moves to two known goal positions, then back to the start. The first two legs of this trajectory are consistent with the robot's model of goal-oriented motion. However, when the human returns to the start, she appears irrational to the robot.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{safety_metric_triangle.png}
    \caption{Safety results for the unmodeled goal scenario.}
    \label{fig:safe_triangle_results}
    %\vspace{-0.9cm}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{efficiency_metric_triangle.png}
    \caption{Efficiency results for the unmodeled goal scenario.}
    \label{fig:eff_triangle_results}
    \vspace{-0.5cm}
    
\end{figure}
Fig.~\ref{fig:safe_triangle_results} and \ref{fig:eff_triangle_results} summarize the performance of the inferred-$\beta$, high-confidence, and low-confidence methods in this scenario. All three methods perform similarly with respect to the minimum distance safety metric in Fig.~\ref{fig:safe_triangle_results}. However, Fig.~\ref{fig:eff_triangle_results} suggests that the inferred-$\beta$ method is several seconds faster than both fixed-$\beta$ approaches. This indicates that, without sacrificing safety, our inferred-$\beta$ approach allows the safe motion planner to find more efficient robot trajectories.






==> (RSS 2018) Quadcopters for the People/intro.tex <==
% To Do:
%%%% Go through PDF of todo changes and check %%%%
% [Jaime][/] Cite Nick Roy (https://doi.org/10.1007/s10514-013-9334-3) -- make it clear that we’re different
% [Jaime][/] In conclusions, mention multiple people
% [Jaime][/] Throw human model xdot = v into running example and note that it is simple
% [Jaime][/] Define the cost. Consider putting a running example after problem formulation

% (done) [Andrea] In conclusions, We used simplest model because want to use simplest model possible to still get decent results. Model will never be perfect. We don’t lose safety by having a bad model, we instead lose effectiveness of plan(?)
% (done) [Andrea] In demo, mention that we use motion capture room. In a realistic application, would need to have other methods for state estimation (e.g. LIDAR)
% (didn't do this, because i dont think reviewer understood) [Andrea] 2) Some symbols are not explicitly defined, such us \tilde{u} in (3), or \hat{\beta}} in (7) and (8).
% [Andrea] Make sure probabilistic safety is clearly defined

% (Add pseudo-code at the end if space)
\blfootnote{This research is supported by an NSF CAREER award, the Air Force Office of Scientific Research (AFOSR), NSF's CPS FORCES and VehiCal projects, the UC-Philippine-California Advanced Research Institute, the ONR MURI Embedded Humans, and the SRC CONIX Center.}
\blfootnote{
    $^*$The first two authors contributed equally to this paper.
}

\section{Introduction}
\label{sec:intro}



%\jfnote{Clarify that for us behavior means motion.}\\
%\jfnote{Provably safe $\to$ probabilistic safety analysis.}\\
%\shnote{TODO: move some beta stuff from prior work into intro to explain confidence bounds}\\
%\shnote{TODO: sort out where to put key insights/contributions}\\

%Robots are becoming increasingly common in daily life, from autonomous drones flying in public spaces to assistive robots helping in the home.\adnote{this past sentence is sugar, and gets stated countless times -- i read it and just think to myself come on, get to the point; suggest delete and start with the next sentence directly} 
In situations where robots are operating in close physical proximity with humans, it is often critical for the robot to anticipate human motion.
%to model the human's motion and predict future movements\adnote{rephrase to the robot needs to anticipate human motion -- don't say the model from the get go, start with something everyone can agree with}. 
%For example, imagine a scenario where a delivery robot is navigating around a person to reach a goal drop-off location (Fig.~\ref{fig:front_fig}). %\abnote{To stay out of the person's way, the robot needs to predict her future movements.
One popular predictive approach is to model humans as approximately rational with respect to an objective function learned from prior data \cite{ ziebart2009planning, kretzschmar2016socially}.
%To stay out of the person's way, the robot can predict the human's future movements by modeling her as approximately rational with respect to an objective learned from prior data \cite{ ziebart2009planning, kretzschmar2016socially}.
    %\adnote{here you're confounding two points --separate them; 1) there is a need for anticipation/prediction; 2) one popular way to achieve this by modeling peole as approximately rational; cite loooots of papers to convey why we are focusing on this particular way of doing it as opposed to others} 
%\adnote{many cites here, e.g. lots of IRL, and then also ziebart pedestrian prediction, kuderer irl social navigation, etc -- just sent you an email with a list}. 
When a person is moving in accordance with the learned objective (e.g. to a known goal location), such models often make accurate predictions and the robot can easily find a safe path around the person.
%When the person is walking directly towards her goal, such models often make the right predictions and the robot can easily find a safe path around the person.
%\adnote{you just started a new idea, so I'd put this last sentence in the next paragraph} 
Unfortunately, no model is ever perfect, and the robot's model of the human will not be able to capture all possible movements that it might eventually observe.
%\adnote{all possible makes it seems like the robot has to do worst case analysis; what you want to say here is that 1) the model will work a lot of the times, but 2) there will be edge cases where it will fail to anticipate how the human actually moves}
For example, the human might walk toward another goal location that the robot does not know about, or move to avoid an obstacle of which the robot is unaware. In these cases where the human's motion diverges from the model's predictions, safety might be compromised. In Fig.~\ref{fig:front_fig} (left), the robot fails to reason about the human avoiding the unobserved obstacle and gets dangerously close to the human.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{RSS_front_figure.pdf}
    \caption{When planning around humans, predictive models can enable robots to reason about future motions the human might take. These predictions rely on human motion models, but such models will often be incomplete and lead to inaccurate predictions and even collisions (left). Our method addresses this by updating its \textit{human model confidence} in real time (right).}
    \label{fig:front_fig}
    \vspace{-.7cm}
\end{figure}

One method to mitigate the effects of model inaccuracy is for the robot to re-compute its human model over time. However, restrictions in sensing and in the availability of human data limit how much a model can be refined online without overfitting. %Additionally, when the ``true'' human objective is outside of the robot's hypothesis space it will never achieve a perfect prediction model.
%Perhaps our human is startled by an angry bee or other ``obstacle" that the robot is not equipped to detect.
% As a result, many robotic systems are likely to benefit from integrating predictive models of human behavior---in particular, human motion---into their motion planning algorithms.
% Recent research has produced predictive models of human motion that allow the robot to find a safe path in \textit{most} situations. 
%COMMENT ADDRESSED -Sylvia
 %\adnote{this previous paragraph would be greatly aided by an example; imagine a robot that needs to navigate around a person; to stay out of the person's way, the robot needs a model of where the person will move next; recently a promising approach emerged to enable this prediction: model the human as being approximately optimal with respect to some objective, learn that objective from prior data; when the person is walking across the room directly towards their goal, this works great (have a fig 1 to point to); but no model is perfect -- what if there is a goal that the robot does not know about, what if there is coffee spilled on the ground and the robot's objective was not trained to know that humans want to not step on stuff that's spilled, what if the robot doesn't have the right sensors to detect an obstacles or has a perception failure; -- give these kinds of examples to show that there is a myriad of things that can go wrong, and most of them would not be solved by relearning the model, the fundamental problem is the space of objectives we're considering}
%NOTE we could change this figure to the one from Jaime's extended abstract for clarity, or explain the current figure more (e.g. where are the humans goals, what is beta?, the scale needs to relate to the probabilities of what?)
Alternatively, the robot can reason about its confidence in its current model's predictions.
In this paper, we propose a method in which the robot continually estimates its confidence in its human model in real time and adapts its motion plan according to this confidence (Fig.~\ref{fig:front_fig}, right).
In particular, our approach leverages the so-called ``rationality'' coefficient in the commonly used Boltzmann model of approximately rational human behavior \cite{baker2007goal,ziebart2008maximum}
%as a single parameter indicating
%- we reason about a single parameter for confidence
%- in this case the parameter is beta which is commonly used...
%
% to treat the ``rationality" coefficient of the human (which regulates the concentration of human action distribution around the predicted
as a time-varying indicator of the model's predictive performance.
This is a single scalar parameter that can
be tractably inferred at deployment time.
% Based on this, the robot can adapt its probabilistic human predictions to account for how well its model is capturing the current behavior.
%
%\adnote{\textbf{very important}: this is NOT a strong contribution in itself; it's crucial here to give the insight of \emph{how} you are getting this estimation; make the following points: 1) to capture the fact that humans aren't perfect, we typically use a rationality coefficient; 2) our observation/insight is that people will take seemingly irrational actions for two reasons -- they are suboptimal, or we don't have the right model, and regardless of which evaluating their apparent irrationality can serve as a natural measure of how confident the robot should be in the model; 3) estimating apparent (ir)rationality online automatically leads to adaptive predictions -- if the person follows the model, the robot's predictions start having lower variance and the robot gets to be more efficient; if the person does not follow the model, then the robot's predictions start having higher variance and the robot becomes more conservative; \textbf{i cannot stress enough the importance of covering points 1-3 above in this introduction}}
%Moreover, the robot should use its prediction model and confidence levels to plan dynamically feasible and safe trajectories in real time.
%
%plan and execute trajectories around the moving human.  Here the robot should account for dynamic feasibility and execution-time tracking inaccuracies to evaluate the risk of collision for the \textit{physical} robot rather than only the often simplified model used for planning.
% Moreover, robots must generate trajectories around humans that are robust and dynamically feasible.
%
% \textcolor{red}{Our insight is that human motion that diverges from the robot's predictions will seem ``irrational'' to the robot.}
%By re-estimating human rationality online, we obtain a confidence estimate for our model that permits the automatic adjustment of future predictions.
We couple the resulting confidence-aware human motion predictions with a provably safe motion planner to obtain \textit{probabilistically safe} robotic motion plans that are conservative when appropriate but efficient when possible.
%When the human's behavior falls outside of the model, predictions will have higher variance and we will naturally obtain more conservative robot behavior in response. Similarly, predictions will have lower variance when the robot gathers enough evidence that the human's behavior fits the model, and we will naturally obtain more efficient robot behavior in response.
%\jfnote{With our proposed method, we have the predictions, and they are uncertain, there's two ways to reason about safety under uncertainty: probability and worst-case.}

\textit{This paper makes two key contributions:}
%\abnote{Claire: be more specific about our technical contributions -- we are learning a single parameter with little data. Use the wording the "adaptive", "online/real time", "when the human's behavior is completely alien to the robot's model, the resulting behavior of the robot is conservative etc.".}
(1) a real-time Bayesian framework for reasoning about the uncertainty inherent in a model's prediction of human movement,
%\adnote{maybe a bayesian framework for adapting the robot's prediction about human motion online based on confidence}
and
(2)~extending a state-of-the-art, provably safe, real-time robotic motion planner to incorporate our time-varying, probabilistic human predictions.
Together, these two contributions facilitate the real-time generation of robot trajectories through human-occupied spaces.
Further, they guarantee that when the robot tracks these trajectories at run-time they will be collision-free with arbitrarily high probability.
% \abnote{
% \begin{itemize}
%     \item learning a single parameter online
%     \item that give us probabilistic predictions 
%     \item which can be used in a robotic motion planner in real time 
%     \item to generate probabilistically safe robot trajectories 
%     \item we use this algorithm to generate trajectories that are provably safe with respect to the physical robotic system 
% \end{itemize}}

%\adnote{i think this could be restated to emphasize the contribution of generalizing guarantees based on the idea of worst-case tracking error to probabilistic dynamic obstacles}\adnote{I also think it's important to call out that the guarantee is over the joint plan+tracking controller, because to a planning community this is pretty interesting, albeit obvious to a controls community}
%COMMENT ADDRESSED -Sylvia
%\adnote{this previous paragraph starts a little little abruptly: want to set up that one option is to reestimate your model, but sometimes you'll just miss the right information, and the  human objective that actually explains the behavior you see will be outside of your hypothesis space; in this paper, we propose that robots should continually estimate their confidence in their human model online, and act more conservatively when they have low confidence; (with this, you're establishing your two goals: estimate confidence, adapt behavior -- that gives you an opportunity to then introduce your key idea that elegantly solves both of them)}
% \adnote{the current intro is very general, and missed the beta estimation as an insight; what we do here is very specific to human models as approximately rational, and that's a good thing -- I think there are probably a bunch of techniques that can estimate confidence in models, and we don't want to compete with that; we also don't want to overclaim -- I doubt we're the first to say that robots should compute confidence in the human models, so that can't be our main thing -- intro needs to get at the core of the paper}
% \adnote{arrive at the key insight for how you are going to have a confidence and adapt the robot's behavior to it; maybe something like "Our key insight is that human behavior that falls outside of our model will seem \emph{irrational} to the robot. By re-estimating human rationality online, we not only get a confidence estimate for our model, but we also automatically adjust future predictions to have higher variance and naturally obtain more conservative robot behavior in response. "}
% \begin{itemize}
%     \item Robots are entering human workspaces
%     \item Even without collaboration, robots need to be able to safely operate around people. 
%     \item Safe operation requires robots to integrate human predictive models into provably safe motion planners. 
%     \item Typically, a good model of human behavior will perform well in \textit{most} situations. 
%     \item Unfortunately, in reality no human model will  be able to capture all possible behaviors the robot might eventually observe. 
%     \item In cases where the structure of the human behavior escapes the model, predictions will generally degrade and safety might be compromised. 
%     \item Even if the robot tries to improve its human model during operation, restrictions in sensing and in the availability of human behavioral data limit how much a model can be refined without incurring overfitting. 
%     \item Rather than attempting to improve the entire model, the robot can reason probabilistically about its confidence in its predictions.  
%     \item In this paper, we argue that robots should validate their human models online and reason about the uncertainty surrounding future predictions in order to produce efficient plans while maintaining safety.
%     \item We make two key contributions: (1) a Bayesian framework for reasoning about the uncertainty inherent in a model's prediction of human behavior, and (2) extending a state-of-the-art, provably safe, real-time robotic motion planner to incorporate our time-varying, probabilistic human predictions.
%     %\item \textit{Insight 1: Robots that reason about the accuracy of their human models are more efficient and can perform more complex/risky maneuvers while still ensuring safety.}
%     %\item \textit{Insight 2: Robots that reason about the ``rationality" of their human model can better react to unmodeled human behaviors.}
%     % OR (2) incorporating time-varying, probabilistic predictions into a state-of-the-art, provably safe, real-time robotic motion planner. 
%     %\item In this paper, we argue that robots should reason about the accuracy of their human models \textit{in real time as they observe actual human behavior} in order to produce efficient plans while maintaining safety. 
%     % keeping track of the observed performance of the model as the human's behavior evolves makes it possible to reason about the uncertainty surrounding future predictions
%     %the model and the uncertainty associated with
%     %\item When robots interact with humans in close physical proximity, modeling human behavior can enable robots to be more efficient and safe when executing a task
%     %\item However, the robot's model of the human is typically pre-defined by the robot designer and may not accurately represent human behavior that the robot actually observes
%     %\item For example, if the robot has high confidence in its model of the human behavior, then it can confidently plan a route nearby the human while still guaranteeing safety. 
%     %\item However, if the human’s behavior does not match the robot’s model very well, then the robot learns to resort to more conservative actions. 
% \end{itemiz

==> (RSS 2018) Quadcopters for the People/notation.tex <==
\newcommand{\pset}{\mathcal{P}} %planner set set
\newcommand{\tset}{\mathcal{S}} %tracker set
\newcommand{\tvar}{t}
\newcommand{\thor}{t_f} % Time horizon
\newcommand{\tstate}{s_R} % Tracker state
\newcommand{\pstate}{x_R} % Planner state
\newcommand{\rstate}{r} % Relative state
\newcommand{\ttraj}{\xi_{\tdyn}} % Tracker trajectory
\newcommand{\ptraj}{\xi_{\pdyn}} %Planner trajectory
\newcommand{\rtraj}{\xi_\rdyn}
\newcommand{\senseDist}{m}
\newcommand{\tctrl}{a_R} % Tracker control
\newcommand{\dstb}{d} % Disturbance
\newcommand{\pctrl}{u_R} % Planner control
\newcommand{\tdyn}{\tilde{h}_R} % Tracker dynamics
\newcommand{\pdyn}{\tilde{f}_R} % Planner Dynamics
\newcommand{\rdyn}{e} % Relative dynamics
\newcommand{\dset}{\mathcal{D}}
\newcommand{\tcset}{\mathcal{U}_s} %tracker control set

==> (RSS 2018) Quadcopters for the People/problem.tex <==
\section{Problem Statement and Approach}
\label{sec:problem}
% ADDRESSED BY JAIME
% \adnote{the structure of this problem statement is a little confusing  -- sometimes too high level, sometimes too low level, and the order is weird in that it doesnt say here is what we know, and then here is our goal, it keeps going back and forth; seems like the problem statement is: there is a robot state, a human state, robot and human actions, dynamics for each; the robot knows human dynamics and has a mdoel of its own dynamics; then the robot has a goal state, and it also has a model of the person as approximately optimizing a reward function (currently equation 4); this model might or might not be accurate; the objective is for the robot to reach its goal (somehow saying a sequence of goals makes it more specific rather than more general), and do it 1) efficiently, and 2) without colliding with the human; this is important because that is the problem you are trying to solve, and you will use these metrics of safety and efficiency later to evaluate how well you are solving it}
% \begin{itemize}
%     \item there is a single robot and single human navigating through same space
%     \item introduce robot state and human state, actions, dynamics
%     \item introduce collision set
%     \item Human want to go to its goal, not cooperating with robot.
%     \item Robot wants to efficiently get to its goal while maintaining safety
%     \item robot has understanding of its goal state(s)
%     \item robot has prediction model of human as approximately optimizing a reward function (eq 4)
%     \item this model may or may not be accurate.  even best possible model may not capture everything (behaviors).
%     \item problem: (1) how do we reason about human prediction model in order to produce probabilistic predictions that account for current confidence in model
%   (2) how do we integrate these predictions with motion planners that can track these trajectories safely and efficiently using realistic quadrotor dynamics?
% \end{itemize}
We consider a single robot moving to a preset goal location in a space shared with a single human, and assume that the human expects the robot to avoid her.
Therefore, it is the robot's responsibility to maintain a safe distance from the human at all times.
We present our theory for a general single human and single robot setting, and use the running example of quadcopter navigating around a walking human to illustrate the proposed approach and demonstrate the utility of our method.

\subsection{Motion Model}
\label{subsec:robot_motion_model}

Let the state of the human be $x_H \in \mathbb{R}^{n_H}$, where $n_H$ is the dimension of the human state space. 
We similarly define the robot's state, for planning purposes, as  $x_R \in \mathbb{R}^{n_R}$.
These states could represent the positions and velocities of a mobile robot and a human in a shared environment or the kinematic configurations of a human and a robotic manipulator in a common workspace.
The human and robot are each modeled by their dynamics:
\begin{equation}
    \begin{aligned}
    \dot{x}_H &= f_H(x_H, u_H) \qquad
    \dot{x}_R &= f_R(x_R, u_R)
    \end{aligned}
\end{equation}
where $u_H \in \mathbb{R}^{m_H}$ and $u_R \in \mathbb{R}^{m_R}$ are the control actions of the human and robot, respectively.

The robot ultimately needs to plan and execute a trajectory to a goal state
according to some notion of efficiency,
while avoiding collisions with the human. %\adnote{we also care about efficiency}
We define the keep-out set $\mathcal{K} \subset \mathbb{R}^{n_H} \times \mathbb{R}^{n_R}$ as the set of joint robot-human states to be avoided, e.g. because they imply physical collisions.
%\remove{For example, in a manipulation task, collision configurations correspond to contact between the human and the robot bodies; in navigation problems, collisions occur when the human and robot move to undesirably close locations.
%In general, the collision set can also contain robot configurations that are unacceptable regardless of the human state (such as collisions with walls or workspace objects).\abnote{OR CUT DOWN}}
To avoid reaching this set, the robot must reason about the human's future motion when constructing its own motion plan.
% \adnote{i am confused by the idea of collision states; do you mean to say that K is the set where human state and robot state are the same? you can write that out explicitly $\{(x_H,X_R)\subset \mathbb{R}^{n_H} \times \mathbb{R}^{n_R} | x_H=X_R\}$; maybe not all state has to be the same -- it's just weird to introduce K and not define it; do you really need it here?} 

%\subsection{Running example}
\example{
We introduce a running example for illustration throughout the paper.
In this example we consider a small quadcopter that needs to fly to locations $g_R \in \mathbb{R}^3$ in a room where a human is walking.
For the purposes of planning, the quadcopter's 3D state is given by its position in space $x_R = [p_x, p_y, p_z]$, with velocity controls assumed decoupled in each spatial direction, up to $v_R=0.25$~m/s.
The human can only move by walking and therefore her state is given by planar coordinates $x_H = [h_x, h_y]$ evolving as $\dot{x}_H = [v_H \cos\phi_H, v_H \sin\phi_H]$.
At any given time, the human is assumed to either move at a leisurely walking speed (${v_H \approx 1}$~m/s) or remain still (${v_H \approx 0}$).
% The quadcopter is assumed to independently control its velocity along each spatial direction, up to $v_R=0.25$~m/s.
% \remove{
%     \begin{subequations}\label{eq:dynamics_plan}
%     \begin{align}
%             &\dot{x}_H = u_H\enspace,\quad
%             u_H\in \{u_H: ||u_H||_2 = v_H\} \cup \{0\}\enspace,\label{eq:dynamics_plan_H}\\
%             &\dot{x}_R = u_R\enspace\,, \quad
%             u_R\in \{u_R: ||u_R||_\infty \le v_R\} \enspace. \label{eq:dynamics_plan_R}
%     \end{align}
%     \end{subequations}
%     }
\\ \indent
In this example, $\mathcal{K}$ consists of joint robot-human states in which the quadcopter is flying within a square of side length $l=0.3$~m centered around the human's location, while at
any altitude, as well as any joint states in which the robot is outside the bounds of a box with a square base of side $L=3.66$~m and height $H=2$~m, regardless of the human's state.
%an altitude lower than $h=2$~m. 
%The human therefore induces a keep-out box of dimensions $l\times l\times h$ in the robot's state space.
% \remove{
% \begin{equation}\label{eq:collision_set}
% \begin{aligned}
%     \mathcal{K} =& \Big\{ (x_R, x_H) : \max\big\{|p_x - h_x|,|p_y - h_y|\big\} \le \frac{l}{2}\Big\} \cup \\
%     &\Big\{ (x_R, x_H) : \max\Big\{\frac{|p_x|}{L},\frac{|p_y|}{L},\frac{|p_z|}{H}\Big\} \ge 1\Big\}
%     \enspace .
% \end{aligned}
% \end{equation}
% In other settings, it may be desirable to impose different keep-out sets, for example forbidding the quadcopter from flying directly in front of people.}
}

\subsection{Robot Dynamics}

Ideally, robots should plan their motion based on a high-fidelity model of their dynamics, accounting for inertia, actuator limits, and environment disturbances.
Unfortunately, reasoning with such complex models is almost always computationally prohibitive.% \todo{is almost always too much?}
 As a result, the models used for planning typically constitute a simplified representation of the physical dynamics of the real robot, and are therefore subject to some error that can have critical implications for safety. In particular, let $s_R\in\mathbb{R}^{n_S}$ denote the state of the robot in the higher-fidelity dynamical model, and let ${\pi:\mathbb{R}^{n_S}\to\mathbb{R}^{n_R}}$ be a known function that projects this higher-fidelity state onto a corresponding planning state, i.e $x_R = \pi(s_R)$. A planner which operates on $x_R$ may generate a trajectory which is difficult to track or even infeasible under the more accurate dynamical model.
Thus reasoning with the planning model alone is not sufficient to guarantee safety for the real robot.
%Section \ref{subsec:fastrack} presents one approach to adress this problem.
%While the robot uses the simplified dynamic model in \eqref{eq:dynamics_plan_R}, its motion is more accurately described by the dynamic model:
%\begin{equation}
%    \dot{s}_R = \tilde{f}_R(s_R,a_R)
%\end{equation}
% As a result, reasoning naively with the planning model is not sufficient to provide safety guarantees for the real robot.

\example{
    We model our quadcopter with the following flight dynamics (in near-hover regime):\\
    \noindent
    \begin{equation}
        \small \label{eq:Quad6D_dyn}
        \begin{bmatrix}
            \dot p_{x}\\ \dot p_{y}\\ \dot p_{z}
        \end{bmatrix}
        = \begin{bmatrix}
            v_{x} \\ v_{y} \\ v_{z} \
        \end{bmatrix}
        \enspace ,\begin{bmatrix}
             \dot v_{x}\\ \dot v_{y}\\ \dot v_{z}\\
        \end{bmatrix}
        = \begin{bmatrix}
              g \tan\theta\\ -g \tan\phi \\ \tau - g 
        \end{bmatrix}
        \enspace,
    \end{equation}
    where $[p_x,p_y,p_z]$ is the quadcopter's position in space and $[v_x,v_y,v_z]$ is its velocity expressed in the fixed world frame, with thrust $\tau$ and attitude angles (roll $\phi$ and pitch $\theta$) as controls.
    %\\ \indent
    The quadcopter's motion planner generates nominal kinematic trajectories in the lower-dimensional $[p_x,p_y,p_z]$ position state space.
    % implicitly using the dynamics in \eqref{eq:dynamics_plan_R}.
    Therefore we have a linear projection map ${\pi(s_R) = [I_3, 0_3] s_R}$, that is, $x_R$ retains the position variables in $s_R$ and discards the velocities.
}

\subsection{Predictive Human Model}

%\jfnote{Introduce Boltzmann model here, without dwelling on model confidence yet.}
%The robot is aware of a predefined set of human behavioral modes, such as possible locations that the human might visit. 
%Importantly, this parametric model will not necessarily capture all types of motion the human can exhibit. 
%This will enable us to study cases when the robot's model of the human does not capture the observed behavior.
%\adnote{since the only model we deal with is the approximately rational model, introduce it here; then leave if for the actual solution to propose reestimating beta to get confidence}
The robot has a predictive model of the human's motion, based on a set of parameters whose values may be inferred under a Bayesian framework or otherwise estimated over time.
Extensive work in econometrics and cognitive science has shown that human behavior can be well modeled by utility-driven optimization \cite{von1945theory, luce1959individual, baker2007goal}.
Thus, the robot models the human as optimizing a reward function, $r_H(x_H,u_H; \theta)$, that depends on the human's state and action, as well as a set of parameters $\theta$. This reward function could be a linear combination of features as in many inverse optimal control implementations (where the weighting $\theta$ between the features needs to be learned), or more generally learned through function approximators such as deep neural networks (where~$\theta$ are the trained weights) \cite{finn2016guided}.

We assume that the robot has a suitable human reward function, either learned offline from prior human demonstrations or otherwise encoded by the system designers. 
With this, the robot can compute the human's policy as a probability distribution over actions conditioned on the state.
Using maximum-entropy assumptions \cite{ziebart2008maximum} and inspiration from noisy-rationality models used in cognitive science \cite{baker2007goal}, the robot models the human as more likely to choose actions with high expected utility, in this case the state-action value (or Q-value):
   \begin{equation}
    \label{eq:observation_model}
        P(u^t_H \mid x^t_H; \beta, \theta) = \frac{e^{\beta Q_H(x^t_H,u^t_H; \theta)}}{\sum_{\tilde u}e^{\beta Q_H(x^t_H,\tilde u; \theta)}}\enspace.
    \end{equation}

\example{
    The quadcopter's model of the human assumes that she intends to reach some target location $g\in\mathbb{R}^2$ in the most direct way possible. The human's reward function is given by the distance traveled $ 
        \label{eq:reward}
        r_H(x_H,u_H;g) = - ||u_H||_2 \enspace$
    and human trajectories are constrained to terminate at $g$.
    The state-action value, parametrized by ${\theta=g}$, captures the optimal cost of reaching $g$ from $x_H$ when initially applying $u_H$:
    $
        \label{eq:value}
        Q_H(x_H,u_H;g) = -||u_H||_2 - ||x_H+u_H-g||_2 .
    $
    }
%\adnote{i think the following stuff is our insight and thus part of our solution, so i'd really move it to the confidence estimation stuff as a first subsection}

The coefficient $\beta$ is traditionally called the \textit{rationality coefficient} and it determines the degree to which the robot expects to observe human actions aligned with its model of utility. 
    %and it determines the concentration of the distribution around the ``optimal human action". 
%\adnote{move everything above to robot's model of human, which is part of the problem statement and not part of our solution -- what we deal with is below, i.e. how to figure out how good this model is online}
A common interpretation of $\beta = 0$ is a human who appears ``irrational," choosing actions uniformly at random and completely ignoring the modeled utility,    while $\beta \rightarrow \infty$ corresponds a ``perfectly rational" human.
%\adnote{I'd move this next sentence to the actual contribution section (IV), and rephrase it; even if people might use it like that, we have to say somewhere that when humans deviate from the model of optimizing the reward, their actions will appear more irrational, and what we propose is to reintrepret beta as model confidence and estimate it online }
Instead, we believe that $\beta$ can be given a more pragmatic interpretation related to the accuracy with which the robot's model of the human is able to explain her motion.
Consistently, in this paper, we refer to $\beta$ as \textit{model confidence}.

Note that we assume the human does not react to the robot. This assumption can realistically capture plausible shared-space settings in which lightweight robots (e.g. micro-drones) may be expected to carry out services such as indoor surveillance in a building while minimizing interference with human activity.
Additionally, to the extent that a more compliant human will tend to avoid collisions with the robot, the robot may still benefit in such scenarios---it is merely not assuming any cooperation \textit{a priori} in its planning.%\adnote{move to discussion? i made a note about that, you can actually stilldo beta estimation if the human reacts... and planning gets harder because of nested otpimizatoin}

\subsection{Probabilistic Safe Motion Planning Problem}
\label{subsec:prob_safe_motion_planning}

The problem that the robot needs to solve is to plan a trajectory that, when tracked by the physical system, will reach a goal state as efficiently as possible while avoiding collisions with high confidence, based on an informed prediction of the human's future motion.

Since any theoretical guarantee is tied to the model it is based on, 
safety guarantees will inherit the probabilistic nature of human predictions.
This induces a fundamental tradeoff between safety and \textit{liveness}:
predictions of human motion may assign non-zero probability to a wide range of states at a future time, which may severely impede the robot's ability to operate in the shared space with ``absolute safety''
(only absolute according to the model).
Therefore, depending on the context, the designers or operators of the system will need to determine what is an acceptable probability that a robot's plan will conflict with the human's future motion.
Based on this, the robot's online planning algorithm will determine when a motion plan is predicted to be \textit{sufficiently safe}. In our demonstrated system, we use a $1\%$ collision probability threshold for planning. 

Our goal now is to find efficient robot motion plans that will keep collisions with a human below an acceptable probability.
Formally, given a current state $x_R^{\text{now}}\in\mathbb{R}^{n_R}$, a cumulative cost ${c:\mathbb{R}^{n_R} \times \mathbb{R}^{m_R} \to \mathbb{R}}$, a probability threshold $P_{\text{th}}\in[0,1]$ and a final time $T$, we define the constrained planning problem:
\begin{subequations}
\begin{align}
        \min_{u_R^{t:T}} &\sum_{\tau=t}^T c(x_R^\tau,u_R^\tau) \label{eq:opt_objective}\\
        \text{s.t. } & x_R^t = x_R^{\text{now}} \label{eq:opt_initial}\\
        &x_R^{\tau+1} = \tilde f_R(x_R^\tau,u_R^\tau), \quad \tau\in{t,...,T-1}\label{eq:opt_dynamics}\\
        & P^{t:T}_\text{coll}:=P\big(\exists \tau\in\{t,...,T\}: \text{coll}(x_R^\tau,x_H^\tau)\big) \le P_{\text{th}}\label{eq:opt_safety}
\end{align}
\end{subequations}
with $\tilde f_R$ a discrete-time approximation of the dynamics~$f_R$. The term $\text{coll}(x_R^t,x_H^t)$ is a Boolean variable indicating whether the human and the robot are in collision.
%\shnote{Jaime thinks we can cut down a lot of the rest of this subsection}
%\adnote{isnt a lot of what follows solution, not problem statement?}
% The key element in our analysis is the safety constraint \eqref{eq:opt_safety}.
% Reasoning about safety of robotic motion in human-robot settings introduces two uncertainty-related challenges that we seek to address in combination.
%
% First, online robotic motion planning requires using simple, tractable models for real-time computation, which unfortunately introduces uncertainty in safety assessment.
%
% If the physical robot was able to exactly follow the motion plan computed through the above optimization, collisions would happen if and only if ${(x_R, x_H) \in \mathcal{K}}$ at any point in time.
% Due to dynamic infeasibility of the generated plan, however, the physical robot may reach a different state, so the real condition for collision is instead ${(\pi (s_R),x_H)\in\mathcal{K}}$.
% Since the planning algorithm cannot tractably plan with the high-fidelity dynamical model of the robot in real time, it cannot explicitly predict $\pi (s_R)$, so collision-checking of candidate plans cannot be done exactly.\abnote{PI IS NOT DEFINED.}
%
% Second, predictions of the human's future state, even when based on well-informed models, may eventually perform poorly when the human's behavior outstrips the model's predictive power.
% In such cases, even a probabilistic model of the human may fail to produce a well-calibrated prediction, which can have a negative impact on the reliability of safety analysis if the model fails to appropriately, and quickly, monitor the confidence of this prediction.
%
The safety analysis necessary to solve this online motion planning problem therefore has two main components, the robot's state and the human's state, both of which are affected by uncertainty in their evolution over time.
We tackle these two sources of uncertainty through a combined method that draws simultaneously on the two main approaches to uncertain systems: probabilistic and worst-case analysis.

\example{
The quadcopter's cost can be a weighted combination of distance traversed and time elapsed on its way to a specified goal: $c(x_R,u_R) = ||u_R||_2 + c_0$.
}

The proposed approach in this paper follows two central steps to provide a quantifiable, high-confidence collision avoidance guarantee for the robot's motion around the human. 
In Section \ref{sec:solution_pred} we present our proposed Bayesian framework for reasoning about the uncertainty inherent in a model's prediction of human behavior. 
Based on this inference, we demonstrate how to generate a real-time probabilistic prediction of the human's motion over time. 
Next, in Section \ref{sec:solution_plan} we introduce a theoretical extension to a state-of-the-art, provably safe, real-time robotic motion planner to incorporate our time-varying probabilistic human predictions yielding a quantitative probabilistic safety certificate.




% The proposed approach in this paper has two central steps. 
% We first construct a real-time prediction of the human's motion, accounting for the current confidence in the model's predictive accuracy. 
% Since this prediction is both dynamic (the human's state is expected to evolve over time) and uncertain (we cannot perfectly determine this evolution), it will induce a time-varying, probabilistic obstacle in the robot's state space. 
% We then feed this prediction into the robot's motion planning logic. 
% In order to ensure safety, we use a planning approach that provides dynamic guarantees at motion execution time.
% %\item FaSTrack uses worst-case analysis to guarantee that the physical robot will remain within a tracking error bound of the planned trajectory.
% % \item We extend FaSTrack to work with probabilistic obstacles by computing the total obstacle probability mass contained in its worst-case tracking error bound.

% Together, these two steps allow us to provide a quantifiable, high-confidence collision avoidance guarantee for the robot's motion around the human. 
% In Section \ref{sec:solution_pred} we present our proposed Bayesian framework for reasoning about the uncertainty inherent in a model's prediction of human behavior. 
% Based on this inference, we demonstrate how to generate a real-time probabilistic prediction of the human's motion over time. 
% Next, in Section \ref{sec:solution_plan} we introduce a theoretical extension to a state-of-the-art, provably safe, real-time robotic motion planner to incorporate our time-varying probabilistic human predictions yielding a quantitative probabilistic safety certificate.

%\adnote{the above is a very nice overview of the entire paper (maybe missing a little substance on the confidence estimation part which is a big deal and cool) -- I wonder since you're separating the confidence/prediction section from the planning section to what extent it might make sense to have the above into the problem statement and rename to "Problem Statement and Summary of the Approach"}


==> (RSS 2018) Quadcopters for the People/related.tex <==
\section{Prior Work}
\label{sec:related}

\subsection{Human Modeling and Prediction}
% \adnote{I (very strongly) think the intro already has to talk about this stuff, i.e. clarify that we focus on models that aprpoximate human as rational; perhaps what should go in this subsection instead should be alternative ways of modeling humans -- at least start with that, and recap from the intro that in this paper we focus on these particular ones because they have showed great awesomeness (low sample complexity, good generalization to new environments)}
% As robots enter shared workspaces with humans, the motion of people becomes a large source of uncertainty for the robot during planning and task execution. Prior work has built on Inverse Reinforcement Learning (IRL) to enable robots to infer human objectives by observing their actions \cite{ng2000algorithms}. In these settings, the robot models the human as taking actions with respect to some unknown reward function and towards some (potentially unknown) goal. The human's actions serve as observations about the true goal and the true reward \cite{ziebart2008maximum}. Typically, it is assumed that the robot knows the set of all possible goals the human could move to as well as all relevant features in the reward a-priori. The robot then only has to infer the relative weighting and likely goal. With this knowledge, the robot can predict future states the human will be in and then plan a path safely around them. \adnote{cut: new intro talks about rational humans, and the story about goals is long and not really necessary}

% In reality, robots will never know all possible goals and features that humans consider when taking actions. Thus, unmodeled human behavior will appear as ``irrational" or sub-optimal to the robot. Even when observing unmodeled behavior, robots using state-of-the-art methods will keep the same confidence in their model of the human, potentially resulting in robot motion plans that conflict with human motion or get unsafely close to the human. In contrast, in this paper we argue that during execution, the robot should use the measurements of human behavior to update its confidence in its own human model.\adnote{also cut: intro already gives examples of this to motivate why we need to estimate confidence} 


% \adnote{instead, talk about human modeling and prediction in general-- here is some good stuff from my review paper, which needs to be rewritten a little (you find the numbered references in the pdf I sent you via email):}


One common approach for predicting human actions is supervised learning, where the current state and the history of the human's actions are used directly to predict future actions. Such approaches have enabled inference and planning around human arm motion \cite{amor2014interaction,ding2011human,koppula2013anticipating,lasota2015analyzing,hawkins2013probabilistic},  navigation \cite{ding2011human}, plans for multi-step tasks like assembly \cite{hawkins2013probabilistic}, and  driving \cite{Schmerling2017}.

Rather than predicting actions directly, an alternative is for the robot to model the human as a rational agent seeking to maximize an unknown objective function. The human's actions up to a particular time may be viewed as evidence about this objective from which the robot may infer the parameters of that objective. Assuming that the human seeks to maximize this objective in the future, the robot can predict her future movements \cite{baker2007goal, ng2000algorithms}. %\cite{bai2015intention, baker2007goal, breazeal2009embodied, bandyopadhyay2013intention, dragan2012formalizing, javdani2015shared, liu2016goal, mainprice2013human, perez2015fast, pellegrinelli2016human, mainprice2015predicting, ng2000algorithms, nguyen2011capir, nikolaidis2015efficient}. This approach has been applied widely across driving, navigation, and manipulation, and teleoperation. 
In this paper, we build on in this work by introducing a principled online technique for estimating confidence in such a learned model of human motion.

%\adnote{call out the difference between producing a probability distribution which is one type of "confidence" and what we do, which is this meta-analysis of the model as a whole does not produce the right probability distribution}
% \shnote{Add this stuff somewhere: Planning based prediction of pedestrians \cite{ziebart2009planning}
%  Unfreezing the Robot (the importance of not treating humans as "immutable" moving obstacles) \cite{trautman2010unfreezing}}
% \abnote{add in work form marco pavone}
%\begin{itemize}
    % \item As robots enter shared workspaces with humans, the motion of people becomes a large source of uncertainty for the robot during planning and task execution. 
    % \item Prior work has built on Inverse Reinforcement Learning (IRL) to enable robots to infer human objectives by observing their actions \cite{ng2000algorithms}. 
    % \item In these settings, the robot models the human as taking actions with respect to some unknown reward function and towards some (potentially unknown) goal. The human's actions serve as observations about the true goal and the true reward \cite{ziebart2008maximum}. 
    % \item Typically, it is assumed that the robot knows the set of all possible goals the human could move to as well as all relevant features in the reward a-priori. The robot then only has to infer the relative weighting and likely goal. With this knowledge, the robot can predict future states the human will be in and then plan a path safely around them. 
    % \item However, in reality, robots will never know all possible goals and features that humans consider when taking actions. Thus, un-modeled human behavior will appear as ``irrational" or sub-optimal to the robot. 
    % \item Even when observing un-modeled behavior, robots using state-of-the-art methods will keep the same confidence in their model of the human, potentially resulting in robot motion plans that conflict with human motion or get unsafely close to the human.   
    % \item  In contrast, in this paper we argue that during execution, the robot should use the measurements of human behavior to update its confidence in its own human model. 
    %\item If the robot observes the human taking ``irrational'' actions, then the robot should be less confident that it's model of the human is accurate, thus leading to more conservative plans. Alternatively, if the robot is very certain that the human's motions match its model, then the robot can take more aggressive maneuvers while still ensuring a collision-free path. 
%     \item Planning based prediction of pedestrians \cite{ziebart2009planning}
%     \item Unfreezing the Robot (the importance of not treating humans as "immutable" moving obstacles) \cite{trautman2010unfreezing}
%     \item end this subsection by saying something about how now we can send robot information about human as an uncertain moving obstacle
% \end{itemize}

\subsection{Safe Robot Motion Planning}
Once armed with a predictive model of the human motion, the robot may leverage motion planning methods that plan around uncertain moving obstacles and generate real-time dynamically feasible and safe trajectories.

%Robust model predictive control can search for trajectories with low collision probability \cite{du2012MPC}, effectively trading off computational complexity for safety. %Alternative methods based on safety funnels \cite{Majumdar2017} and contraction-mapping techniques \cite{Singh2017} can also provide robust guarantees for robots with complicated dynamics.
To avoid moving obstacles in real time, robots typically employ reactive and/or path-based methods. Reactive methods directly map sensor readings into control, with no memory involved \cite{belkhouche2009reactive}. Path-based methods such as rapidly-exploring random trees and A* find simple kinematic paths through space and, if necessary, time \cite{hart1968astar,karaman2011RRTPRM}.
% \adnote{do we need to cite that paper Jaime dug up, Schmerling2017, for how they do planning with the prediction?}
% \jfnote{Yes, I had written up a paragraph, not sure where it went!}
These path-based methods of planning are advantageous in terms of efficiency,
yet, while they have in some cases been combined with probabilistically moving obstacles \cite{Aoude2013probabilistically,ziebart2009planning},
they do not consider the endogenous dynamics of the robot or exogenous disturbances such as wind. As a result, the robot may deviate from the planned path and potentially collide with obstacles. It is common for these plans to try to avoid obstacles by a heuristic margin of error. FaSTrack is a recent algorithm that provides a guaranteed tracking error margin and corresponding error-feedback controller for dynamic systems tracking a generic planner in the presence of bounded external disturbance \cite{herbert2017fastrack, fridovich2018planning}. Our work builds upon FaSTrack to create an algorithm that can safely and dynamically navigate around uncertain moving obstacles in real time.

% \jfnote{HIGHLY RELEVANT from Marco: \textit{Multimodal Probabilistic Model-Based Planning for Human-Robot Interaction} They seem to essentially update $\theta_H$, as in Anca's above comment, so we should definitely cite them as a key reference.}\adnote{nice find!}
% \remove{Finally, recent work uses conditional variational autoencoder neural networks inspired by natural language prediction to directly learn probability distributions over human responses from a corpus of human-human interactions, and combines the learned predictive model with model-based motion planning \cite{Schmerling2017}.
% %\adnote{this seems like it fits in the directly prediction actions, not modeling people as rational; so it should go in maybe the top section on prediction actions directly}
% The authors apply this method to interactive autonomous driving simulation achieving state-of-the-art results.}
% Our proposed approach is meant to be complementary to these techniques, allowing robots to quickly notice and adapt to declines in prediction reliability, such as performance degradation when observed driver behavior significantly departs from the training dataset.
% While the concrete method presented in this paper applies exclusively to model-based human predictions, we envision extending it to a more general class of probabilistic predictive models.\adnote{not sure this is right in that we don't really focus on non-rational models of humans, where you have a neural net predict a distribution; confidence in nn predictions is a whole different game}



%Once the robot has a local estimate of the environment, including an understanding obstacles and the movement of humans, it needs to generate and follow a trajectory to its goal while maintaining safety. The robot must satisfy the following challenges: 1) planning in real time, 2) planning around uncertain moving obstacles, 3) generating dynamically feasible trajectories, and 4) being robust to external disturbances (e.g. wind).

%To accomplish challenge 1 and operate in real-time, many planners make simplifying assumptions about the robot's dynamics. With uncomplicated models, techniques like linear model predictive control (MPC) \cite{richter2012realtimeMPC} can operate efficiently. Even more computationally efficient are planners like rapidly-exploring random trees (RRT), progabilistic roadmaps (PRM), and A*; these planners quickly generate basic kinematic paths through the environment \cite{karaman2011RRTPRM}, \cite{hart1968astar}. If the search space is augmented through time, simple trajectories around moving obstacles can be found. However, these methods do not account for the internal dynamics of the robot, and additionally are not typically robust to external disturbances. As a result, the robot may often unsafely deviate from the planned trajectory while moving through the space, potentially colliding with obstacles. Therefore, these methods satisfy challenges 1 and 2, but not 3 and 4.

%When safety is critical, methods that plan with more realistic dynamics are employed. Nonlinear tube MPC
%begin{itemize}
%    \item Other methods \textbf{(cite robust/tube mpc, reachability, etc.)} can plan with more realistic dynamics around moving obstacles, but are generally too slow for real-time implementation.
%    \item When operating around humans, ensuring that the robot plans quickly but also safely is particularly important. 
%    \item FaSTrack is a method that allows for real-time planning using a simplified system model, while simultaneously tracking this plan with the robotic system \cite{herbert2017fastrack, fridovich2018planning}. Tracking error bounds paired with a feedback controller based on relative state between the true system and the plan together guarantee safety of the robot. FaSTrack can be used with time-varying planners, and also can account for bounded external disturbances. Therefore, FaSTrack addresses all four challenges and allows our robot to quickly and safely navigate around the moving human.
%\end{itemize}


==> (RSS 2018) Quadcopters for the People/solution.tex <==
\section{Confidence-Aware Human Motion Prediction}

\label{sec:solution_pred}
%\adnote{seems like you have a separate section for planning (and tracking), so stick to confidence estiamtion for this section title}


%\subsection{Reasoning about Confidence in Human Predictions}

Predictions of human motion, even when based on well-informed models, may eventually perform poorly when the human's behavior outstrips the model's predictive power.
Such situations can have a negative impact on safety if the robot fails to appropriately, and quickly, notice the degradation of its predictions.
%Particularly,
%of attributing the mismatch to the human's rationality,
%in the context of robotics we believe that this mismatch often indicates a modeling error on the robot's side.
%In other words, the robot's model of the human is not rich enough to correctly explain the human's actions.

It will often be the case in practice that the same model will perform variably well over time in different situations and for different people. In some cases this model might be perfectly representative, in others the robot might not have access to some important feature that explains the human's behavior, and therefore the robot's conservativeness should vary accordingly. 


Given a utility-based human model in the form of \eqref{eq:observation_model}, the $\beta$ term can be leveraged as an indicator of the model's predictive capabilities, rather than the human's actual level of \textit{rationality}.
%\adnote{now is a good time to introduce the key to making it all work: reinterpet beta; something like this: "\emph{We obtain this adaptive conservativeness by reinterpreting the rationality coefficient $\beta$ as a measure of \emph{confidence in the robot's model in the human}}. The reason why this works is that when humans do not fit the robot's assumption that they are rational with respect to some reward (either because they are suboptimal, or because they care about some unobserved feature), their actions are going to seem irrational. By maintaining an online estimate of $\beta$, the robot can dynamically adapt its predictions ...."}
Thus, by maintaining an estimate of $\beta$, the robot can dynamically adapt its predictions (and therefore its motion plan) to the current reliability of its human model.
For this reason, in this paper, we refer to $\beta$ as \textit{model confidence},
and aim to make the robot reason about its value in real time in order to generate confidence-aware ``introspective" predictions of the human's motion.

\subsection{Real-time Inference of Model Confidence}
At every time step $t$, the robot obtains a new measurement%
\footnote{In practice, the robot measures the evolution of the human state and computes the associated action by inverting the motion model.}
of the human's action, $u^t_H$. This measurement can be used as evidence to update the robot's belief $b^t(\cdot)$ about $\beta$ over time via a Bayesian update:
    \begin{equation}
    \label{eq:belief_update}
        b^{t+1}(\beta) = \frac{P(u^t_H \mid x^t_H; \beta, \theta)b^{t}(\beta)}{\sum_{\hat\beta} P(u^t_H \mid x^t_H; \hat\beta,\theta)b^{t}(\hat\beta)} \enspace ,
    \end{equation}
    with $b^t(\beta) = P(\beta| x_H^{0:t})$ for $t\in\{0,1,...\}$, and ${P(u^t_H | x^t_H; \beta, \theta)}$ given by \eqref{eq:observation_model}.
It is critical to be able to perform this update extremely fast, which would be difficult to do in the original continuous hypothesis space $\beta\in[0,\infty)$ or even a large discrete set.
Fortunately, as we will see in Section~\ref{sec:demo}, maintaining a Bayesian belief over a relatively small set of $\beta$ values ($N_\beta\approx10$ on a log-scale) achieves significant improvement relative to maintaining a fixed precomputed value.%
\footnote{
Since the predictive performance of the model might change over time as the human's behavior evolves,
%we want to allow the possibility that $\beta$ will also change over time.
%To do this,
we do not in fact treat $\beta$ as a static parameter, but as a hidden state in a hidden Markov model (HMM).
Concretely, between successive ``measurement updates" \eqref{eq:belief_update}, we apply a uniform smoothing ``time update", allowing our belief over $\beta$ to slowly equalize over time, which has the effect of downweighting older observations.
}
% \begin{equation}
%     \label{eq:time_update}
%     b(\beta'|\beta) =
%     \begin{cases}
%         1-\epsilon &\text{if } \beta'=\beta\\
%         \frac{\epsilon}{N_\beta-1} &\text{if } \beta'\neq\beta
%     \end{cases}
% \end{equation}
% with $\epsilon$, typically set to a small value.

%\adnote{people will wonder how the heck we do this online, since 1) its a continuous nongussian distribution, and 2) more importantly, the probability distribution over human actions depends on q function -- worth explaining a little bit and acknowledging limitations, maybe pointing to what to do in high dim like MLE estimate with laplace approx of the partition function, an analogous to e.g. sergey's local ioc paper}
\subsection{Human motion prediction}
We can now use the belief over $\beta$ to recursively propagate the human's motion over time and obtain a probabilistic prediction of her state at any number of time steps %$\delta$
into the future.
In particular, at every future time step, we can estimate the likelihood of the human taking action $u_H$ from any state $x_H$ by directly applying \eqref{eq:observation_model}.
Combining this with the dynamics model, we can generate a distribution of human occupancies over time, with the recursive update:
    \begin{equation}\label{eq:pred_recursive}
    \begin{split}
        % P(&x_H^{t+\delta} \mid x_H^{t};\beta,\theta) =\\
        % &\sum_{x_H^{t+\delta-1}}P(x_H^{t+\delta} \mid x_H^{t+\delta-1};\beta,\theta)P(x_H^{t+\delta-1} \mid x_H^{t};\beta,\theta)
        P(&x_H^{\tau+1} \mid x_H^{\tau};\beta,\theta) =\\
        &\sum_{u_H^{\tau}}P(x_H^{\tau+1} \mid x_H^{\tau},u_H^{\tau};\beta,\theta)P(u_H^\tau \mid x_H^{\tau};\beta,\theta) \enspace ,
    \end{split}
    \end{equation}
     for $\tau\in\{t,...,T\}$;
     % t+\delta-1\}$;
     for the deterministic dynamics in our case, $P(x_H^{\tau+1} \mid x_H^\tau, u_H^\tau;\beta, \theta)=\mathds{1}\{x_H^{\tau+1}=\tilde f_H(x_H^\tau,u_H^\tau)\}$. %\remove{The above transition probability is obtained as:
%     \begin{equation}
%     \begin{split}
%         P(x_H^{\tau}& \mid x_H^{\tau-1};\beta,\theta) = \\
%         &P(x_H^{\tau} \mid x_H^{\tau-1}, u_H^{\tau-1}) P(u^t_H \mid x^t_H; \beta, \theta) \enspace .
%     \end{split}
%     \end{equation}
% While this probability distribution is well-defined for a continuous state space, in practice we approximate it with a probabilistic occupancy grid.
% Since we have deterministic dynamics, $P(x_H^{\tau} \mid x_H^{\tau-1}, u_H^{\tau-1}) = \delta(x_H^{\tau}, f(x_H^{\tau-1}, u_H^{\tau-1}))$, where $\delta(\cdot,\cdot)$ is the delta distribution (this is Dirac's delta for our continuous state space, and Kronecker's delta on the corresponding discretized grid). \abnote{necessary or nah?}}\\

\example{
    \begin{figure}
    \includegraphics[width=.48\textwidth]{coffee_six.pdf} 
    \caption{Snapshots of human trajectory and probabilistic model predictions. Top row: Human moves from the bottom right to a goal marked as a red circle. Bottom row: Human changes course to avoid a spill on the floor. The first two columns show the predictions for low and high model confidence; the third column shows the predictions using our Bayesian model confidence.}%\adnote{annotate with beta estimate? if too hard because it's a distribution, maybe annotate with text like "confident initially", "uncertain" etc}
    \vspace{-0.5cm}
    \label{fig:coffee_six}
    \end{figure}
    % The quadcopter's model of the human considers a number of known frequently-visited locations $\theta\in\{g_1,...,g_N\}$ that she might intend to walk to next; for now, we will let the robot assume that the human is heading to $\theta = g_1$.
    % it expects that the human will move towards her current goal in the most direct way possible.
    %\abnote{Add in simulation of prediction with $\beta$ and without (e.g. two goals and human is going in between)}.
    %If the robot models the human as having an intended goal $g$ \adnote{the goal is a little distracting because it suggests that the goal is the mismodelled part, when perhaps the most realistic example is the coffee one where the human cares about features that the robot does not access} 
    The simplest scenario in our running example involves a human moving towards a known goal. In Fig \ref{fig:coffee_six}(a-c), the human acts predictably, moving directly to the goal. Each subfigure shows the robot's human prediction under different confidence conditions. Predictions for the second scenario, where the human deviates from her path to avoid a coffee spill on the ground, are shown in Fig \ref{fig:coffee_six}(d-f).
    %
    %As the human's trajectory deviates from the goal, the robot's confidence in the predicted model decreases with more probability being assigned to lower confidence values.\adnote{the human does not deviate from g, but rather deviates from the reward function that the robot is assuming? because they go to g, but care about an additoinal feature?}
    % Even if we don't do this right away, we should have
    }


% \begin{figure}[t!]
% \subfigure[Multiple snapshots of a human's trajectory, starting at the green marker, and the corresponding predictions with model confidence inference. Model prediction matches well with the human motion while the human is moving towards the goal, so the uncertainty decreases. As the human turns away from the goal, the uncertainty grows, as the model is less able to explain the observed behavior.  \label{fig:beta}]{\includegraphics[width=.5\textwidth]{figs/beta3.pdf}}\hfill
% \subfigure[Model predictions \textit{without} model confidence inference. The model confidently predicts the human's towards the goal as she approaches it, but continues to predict with confidence that she will return towards the modeled goal even when she veers past it. \jfnote{Arrows in the direction of predicted motion might help here} \label{fig:nobeta}]{\includegraphics[width=.5\textwidth]{figs/nobeta3.pdf}}
% \caption{The start of human trajectory is shown as a green sphere. A single goal location is known modeled beforehand and denoted by red sphere. The red rectangle represents the measured human position as they move in an unexpected arc motion through the space.  \abnote{for final figures, add in the probability color scale (yellow = low prob, pink = high prob?)}} \label{fig:beta_estimation}
% \end{figure}


\subsection{Integrating Model Confidence into Online Model Updates}

When a robot is faced with human behavior that is not well explained by its current model, it can attempt to update some of its elements to better fit the observed human actions.
These elements can include parameters, hyperparameters, or potentially even the structure of the model itself. 
Assuming that the parameters can be tractably adjusted online, this update may result in better prediction performance.
% Nevertheless, there will always be aspects of the observed behavior that were not encoded in the structure of the model to begin with. That is, no single set of values for the parameters would suffice to explain the observed behavior.

% In contrast to parameter adjustments, updating the structure of the model online from the observed human behavior is often computationally infeasible.
% Even in cases where the structure can be changed during the robot's operation, it is still unrealistic to assume that the updated model will explain all future unseen behavior, particularly given the risk of overfitting to prior observations. Therefore,
Even under online model updates, it continues to be necessary for the robot to reason about model confidence.
In this section we demonstrate how reasoning about model confidence can be done compatibly (and in some cases jointly) with model parameter updates. %It may often be the case that what the human cares about is outside of the space of possible new models the robot is considering, because the robot does not have access to all the relevant information. Therefore, updating the model in those situations could result in a slightly more accurate model, but could also give the robot false confidence by locally explaining the human's behavior under the wrong hypothesis, leading to confident but incorrect predictions a few moments later.

% overfit to some particular sequence of actions that could be explained by a hypothesis, and cause the robot to be too confident as the task progresses; for example, if the human is avoiding an unknown obstacle the robot might wrongly update its model to think the human is going to a different goal, and then make wrong confident predictions a few steps later.


Recall that $\theta$ denotes the set of parameters in the human's utility model. The ideal approach is to perform inference over both the model confidence, $\beta$, and the model parameters, $\theta$ by maintaining a joint Bayesian belief, $b^t(\beta, \theta)$. 
The joint Bayesian belief update rule takes the form
\begin{equation}
    b^{t+1}(\beta,\theta) = \frac{P(u^t_H \mid x^t_H; \beta, \theta)b^t(\beta, \theta)}{\sum_{\hat{\beta}, \hat{\theta}} P(u^t_H \mid x^t_H; \hat{\beta}, \hat{\theta})b^t(\hat{\beta}, \hat{\theta})}
    \enspace ,
\end{equation}
with $b^t(\beta,\theta) = P(\beta,\theta \mid x^{0:t}_H, u^{0:t}_H)$.%
\footnote{
Analogously to the case with $\beta$-only inference, the parameters $\theta$ can be allowed to evolve as a hidden state.
}
This approach can be practical for parameters taking finitely many values from a discrete set, for example, possible distinct modes for a human driver (distracted, cautious, aggressive).

\example{
The quadcopter's model of the human considers a number of known frequently-visited locations $\theta\in\{g_1,...,g_N\}$ that she might intend to walk to next.
However, there may be additional unmodeled destinations, or more complex objectives driving the human's motion in the room (for example, she could be searching for a misplaced object, or pacing while on the phone). Fig. \ref{fig:triangle_three} shows how reasoning about model confidence \textit{as well as} the human's destination enables the robot to navigate confidently while the human's motion is well explained by the model, and automatically become more cautious when it departs from its predictions. More detailed results are presented in Section~\ref{sec:demo}.
}

For certain scenarios or approaches it may not be practical to maintain a full Bayesian belief on the parameters, and these are instead estimated over time (for example, through a maximum likelihood estimator (MLE), or by shallow re-training of a pre-trained neural network). In these cases, a practical approach can be to maintain a ``bootstrapped" belief on $\beta$ by running the Bayesian update on the running parameter estimate $\bar\theta$:
    \begin{equation}
        \label{eq:bootstrap}
        \bar{b}^{t+1}(\beta) = \frac{P(u^t_H \mid x^t_H; \beta, \bar{\theta})\bar{b}^{t}(\beta)}{\sum_{\hat\beta} P(u^t_H \mid x^t_H; \hat\beta,\bar{\theta})\bar{b}^{t}(\hat\beta)}
        \enspace .
    \end{equation}
    % \end{remark}
\example{
The quadcopter's predictions of human motion are parameterized by her walking speed $v_H$;
the quadcopter maintains a simple running average based on recent motion-capture measurements,
and incorporates the current estimate into inference and prediction.
}

When it is not desirable or computationally feasible to update the parameter estimate $\bar{\theta}$ continually, we can leverage our model confidence as an indicator of when re-estimating these parameters may be most useful---namely as confidence in the model under the current parameter estimates degrades.

%\adnote{I think I like this running example thing! It's also nicely separated so I can skip it easily if I don't care}

    \begin{figure}
\includegraphics[width=.48\textwidth]{triangle_three.pdf} 
\caption{In this example the human is moving in a counter-clockwise motion to two goals (marked in red), and then to a third unknown goal (located at the same position as the start). Subfigures (a) and (b) show the predictions for a low and high $\beta$, respectively.
%shows the predictions for a low $\beta$, where the robot is always uncertain. Subfigure (b) and shows the predictions for a high $\beta$, where the robot assumes the human will always navigate toward a known goal, even when she is moving in the opposite direction. 
Subfigure (c) shows the predictions using our inferred model confidence, where the robot is confident when the human is moving ``rationally'', and uncertain when the human behavior does not match the robot's model.}
\label{fig:triangle_three}
\vspace{-0.7cm}
\end{figure}


\section{Safe Probabilistic Planning and Tracking} \label{sec:solution_plan}

Once it can generate real-time probabilistic predictions of the human's motion, the robot needs to plan a trajectory that will, with high probability, avoid collisions with her.
On the one hand, any rigorous safety analysis for a robotic system needs to account for deviations of the actual dynamic trajectory from the ideal motion plan.
On the other hand, since human motion predictions are by nature uncertain, the safety analysis will necessarily be quantified in probabilistic terms.
To this end, we build on the recent FaSTrack framework \cite{herbert2017fastrack}, which provides control-theoretic robust safety certificates in the presence of deterministic obstacles, and extend the theoretical analysis to provide probabilistic certificates allowing uncertain dynamic obstacles (here, humans). 

\subsection{Background: Fast Planning, Safe Tracking}
\label{subsec:fastrack}
% \adnote{call this background in the title to differentiate from the other sections which are novel?}
Recall that $x_R$ and $u_R$ are the robot's state and control input, for the purposes of motion planning.
% These models typically constitute a simplified representation of the physical dynamics of the real robot, and are therefore subject to some error that can have critical implications in ensuring safety.
The recently proposed FaSTrack framework \cite{herbert2017fastrack} uses Hamilton-Jacobi reachability analysis~\cite{Evans1984,Mitchell2005} to provide a simple real-time motion planner with a worst-case tracking error bound and error feedback controller for the dynamic robot.
%to guarantee that the physical robot will remain within a tracking error bound of a planned trajectory, even when this plan was generated using a simpler motion model to keep computation tractable in real time.
%The tracking error certificate provided by FaSTrack is based on Hamilton-Jacobi reachability analysis~\cite{Evans1984,Mitchell2005}, which provides %The robust bound is obtained by solving a differential pursuit-evasion type game between the physical robot's controller and an adversarial planner that will generate the hardest possible plan to track, effectively trying to ``escape'' from the robot.
%The solution to this game gives 
%the optimal tracking strategy for the robot, as well as the worst-case error that can ever be reached relative to the planner's reference, as long as the tracking controller plays this optimal strategy.
% In particular, let $s_R\in\mathbb{R}^{n_H}$ denote the state of the robot in the higher-fidelity dynamical model, and let $M\in\mathbb{R}^{n_R\times n_H}$ be a known matrix that projects this higher-fidelity state onto the equivalent planning state, i.e $x_R = \pi (s_R)$.
Formally, FaSTrack precomputes an optimal tracking control policy, as well as a corresponding compact set $\mathcal{E}$ in the robot's planning state space, such that ${\big(\pi (s_R^t) - x_{R,\text{ref}}^t\big)\in \mathcal{E}}$ for \textit{any} reference trajectory proposed by the lower-fidelity planner.
This bound $\mathcal{E}$ is a trajectory tracking certificate that can be passed to the online planning algorithm for real-time safety verification:
the dynamical robot is guaranteed to \textit{always} be somewhere within the bound relative to the plan.
Therefore the planner can generate safe plans by ensuring that the entire bound around the nominal state remains collision-free throughout the trajectory.
Note that the planner only needs to know $\mathcal{E}$ and otherwise requires no explicit understanding of the high-fidelity model.

\example{
    Since dynamics \eqref{eq:Quad6D_dyn} are decoupled in the three spatial directions,
    the bound $\mathcal{E}$
    computed by FaSTrack
    is an axis-aligned box of dimensions  $\mathcal{E}_x \times \mathcal{E}_y\times \mathcal{E}_z$.
}
    % The physical quadcopter in our demonstrations is a Crazyflie 2.0, modeled by the following flight dynamics (in near-hover regime):\\
    % \noindent
    % \begin{equation}
    %     \small \label{eq:Quad6D_dyn}
    %     \left[ \begin{array}{c}
    %         \dot p_{x}\\ \dot p_{y}\\ \dot p_{z}\\ \dot v_{x}\\ \dot v_{y}\\ \dot v_{z}\\
    %     \end{array} \right]
    %     = \left[ \begin{array}{c}
    %         v_{x} \\ v_{y} \\ v_{z} \\ g \tan\theta\\ -g \tan\phi \\ T - g 
    %     \end{array} \right]
    %     \enspace ,
    % \end{equation}
    % where $[p_x,p_y,p_z]$ is the quadcopter's position in space and $[v_x,v_y,v_z]$ is its velocity expressed in the fixed world frame.
    % Lightweight quadcopters commonly accept thrust $T$ and attitude angles (roll $\phi$ and pitch $\theta$) as over-the-air inputs to their on-board controller.
% \\ \indent
% \example{
%     To account for the unmodeled dynamics---%
%     such as rotational inertia and aerodynamic effects,
%     as well as possible time delays and inaccuracies in the low-level control loop---%
%     FaSTrack additionally considers a worst-case additive disturbance affecting the state derivative.
%     \\ \indent
%     % The quadcopter is tracking a nominal trajectory planned using space-time A* \cite{hart1968astar} on a grid discretization of the 3D position state space.
%     % Implicitly, the planner is using the dynamics in \eqref{eq:dynamics_plan_R}:
%     % \begin{equation}
%     %     \small \label{eq:Quad3D_dyn}
%     %     \left[ \begin{array}{c}
%     %         \dot{p}_{x}\\ \dot{p}_{y}\\  \dot{p}_{z}\\
%     %     \end{array} \right] =
%     %     \left[ \begin{array}{c} u_x\\ u_y\\ u_z\\ \end{array} \right ]
%     %     \enspace ,
%     % \end{equation}
%     % with $u_R=[u_x,u_y,u_z]$.
%     % Therefore in this case $M = [I_3, 0_3]$, that is, $x_R$ retains the position variables in $s_R$ and discards the velocities.
%     The dynamics in \eqref{eq:Quad6D_dyn} are decoupled between the three spatial directions, and the resulting tracking error bound $\mathcal{E}$ is a 3D box in the quadcopter's position space \cite{herbert2017fastrack}.
% }

\subsection{Robust Tracking, Probabilistic Safety}
%\adnote{perhaps we can give a little more structure to this subsection to guide the reader by using noindent textbf or paragraph -- perhaps formulation of probabilistic safety, and then proposed approximation}

Unfortunately, planning algorithms for collision checking against deterministic obstacles cannot be readily applied to our problem.
Instead, a trajectory's collision check should return the probability that it \textit{might} lead to a collision.
Based on this probability, the planning algorithm can discriminate between trajectories that are \textit{sufficiently safe} and those that are not.

% Since any theoretical guarantee is tied to the model it is based on
% safety guarantees will inherit the probabilistic nature of human predictions.
% This induces a fundamental tradeoff between safety and \textit{liveness}:
% predictions of human motion may assign non-zero probability to a wide range of states at a future time, which may severely impede the robot's ability to operate in the shared space with ``absolute safety''
% (only absolute according to the model).
% Therefore, depending on the context, the designers or operators of the system will need to determine what is an acceptable probability that a robot's plan will conflict with the human's future motion.

% Our goal is therefore to find efficient robot motion plans that will keep collisions with a human below an acceptable probability.
% Formally, given an initial state $x^i\in\mathbb{R}^{n_R}$, a cumulative cost ${c:\mathbb{R}^{n_R} \times \mathbb{R}^{m_R} \to \mathbb{R}}$, a probability threshold $P_{\text{th}}\in[0,1]$ and a time horizon $T$, we can define the constrained planning problem:
% \begin{subequations}
% \begin{align}
%     \label{eq:opt}
%         \min_{u_R^{0:T}} &\sum_{t=0}^T c(x_R^t,u_R^t) \label{eq:opt_objective}\\
%         \text{s.t. } & x_R^0 = x^i \label{eq:opt_initial}\\
%         &x_R^{t+1} = f_R(x_R^t,u_R^t), \quad t\in{0,...,T-1}\label{eq:opt_dynamics}\\
%         & P^{0:T}_\text{coll}:=P\big(\exists t\in\{0,...,T\}: \text{coll}(x_R^t,x_H^t)\big) \le P_{\text{th}}\label{eq:opt_safety}
% \end{align}
% \end{subequations}
% The term $\text{coll}(x_R^t,x_H^t)$ is a Boolean variable indicating whether the human and the robot are in collision.
% If the physical robot was able to follow the plan exactly, collisions would happen if and only if ${(x_R, x_H)\in\mathcal{K}}$.
As discussed in Section~\ref{subsec:prob_safe_motion_planning}, a safe online motion planner should continually check
the probability that, at any future time $\tau$,
%whether 
${(\pi (s_R^\tau),x_H^\tau)\in\mathcal{K}}$.
%while planning online.
%rather than the naively reasoning about a motion plan's collisions by checking whether ${(x_R,x_H)\in\mathcal{K}}$,
%a safe motion planner should acknowledge that, at trajectory execution time,
% However, due to tracking inaccuracies, 
%While the planning algorithm cannot tractably plan with the high-fidelity dynamical model of the robot, and therefore, cannot explicitly compute $\pi (s_R)$ at any given time, 
The tracking error bound guarantee from FaSTrack allows us to conduct worst-case analysis on collisions given a human state $x_H$:
if no point in the Minkowski sum $\{x_R+\mathcal{E}\}$ is in the collision set with $x_H$, we can guarantee that the robot is not in collision with the human.
%, \remove{that is:
%\begin{equation} \label{eq:worst_case_safety}
%  \big((\tilde{x}_R,x_H)\not\in\mathcal{K}, \; \forall \tilde{x}_R \in \{x_R+\mathcal{E}\}\big) \Rightarrow \big(\pi (s_R), x_H\big)\not\in\mathcal{K}
%  \;%\enspace
%  .
%\end{equation}}

The probability of a collision event for any point $x_R^\tau$ in a candidate trajectory plan, assuming worst-case tracking error, can be computed as the total probability that $x_H^\tau$ will be in collision with \textit{any} of the possible robot states $\tilde{x}_R\in\{x_R^\tau+\mathcal{E}\}$.
For each robot planning state $x_R\in\mathbb{R}^{n_R}$ we can define the set of human states in potential collision with the robot:
%under worst-case tracking:
%\jfnote{Give this guy an intuitive short name.}
\begin{equation}\label{eq:H_E}
   \mathcal{H}_\mathcal{E}(x_R) := \{ \tilde{x}_H\in\mathbb{R}^{n_H}: \exists \tilde{x}_R\in\{x_R+\mathcal{E}\}, (\tilde{x}_R,\tilde{x}_H)\in\mathcal{K} \}
   \enspace .
\end{equation}
The following result is then true by construction.

%\abnote{Claire: Make this proposition bold.}
%\begin{proposition}
\textbf{{Proposition 1:}}\emph{
    The probability of a robot with worst-case tracking error $\mathcal{E}$ being in collision with the human at any trajectory point $x_R^\tau$ is bounded above by the probability mass of $x_H^\tau$ contained within $\mathcal{H}_\mathcal{E}(x_R^\tau)$.
    }
%\end{proposition}
%\jfnote{Insert Running example here to give intuition.}
% In order to reason probabilistically about the safety of a motion plan, we can then combine the worst-case error bound from FaSTrack with the probabilistic human prediction by computing the total probability mass contained inside the tracking error bound.
%To maintain safety with respect to the human, we introduce a probabilistic collision checker that combines the worst-case tracking error bound and the probabilistic human prediction.

Therefore,
% under worst-case tracking error $\mathcal{E}$,
the left-hand side of the inequality in our problem's safety constraint \eqref{eq:opt_safety} can be rewritten as 
%\begin{equation}
%        P^{0:T}_\text{coll}=P\big(\exists t\in\{0,...,T\}, x_H^t\in \mathcal{H}_\mathcal{E}(x_R^t)\big) \le P_{\text{th}}
        %\enspace
%\end{equation}
%The left-hand-side probability is equal to the expression
\begin{equation}
    P^{t:T}_\text{coll} = 1-\prod_{\tau=t}^T P\big(x_H^\tau\not\in \mathcal{H}_\mathcal{E}(x_R^\tau)
    \mid x_H^\tau\not\in \mathcal{H}_\mathcal{E}(x_R^s), t\le s<\tau\big) %\le\\ P_{\text{th}
    %\enspace
    .
\end{equation}

Evaluating the above probability exactly would require reasoning jointly about the distribution of human states over all time steps, or equivalently over all time trajectories $x_H^{0:T}$ that the human might follow.
%Even under state-space discretization, computing this distribution is highly intractable, given that the size of the hypothesis space scales exponentially with $T$.
Due to the need to plan in real time, we must in practice approximate this distribution.%Since our intention is to incorporate this reasoning into the collision-checking step for the robot's real-time motion planner (which will typically need to perform thousands of checks in a fraction of a second), we instead need to approximate this distribution.

%\remove{At first, one might consider assuming independence of all human state predictions at each time step and compute the product of marginal probabilities $P\big(x_H^t\not\in \mathcal{H}_\mathcal{E}(x_R^t)\big)$, usually termed a ``noisy OR'' operation.
%However, given that these marginal time predictions are generated recursively from each other through \eqref{eq:pred_recursive}, this is clearly a highly inaccurate assumption.
%In addition, this approximation will tend to be unreasonably conservative, since the positive correlation emerging from continuity of human trajectories implies that the probability of a robot trajectory not colliding with the human at time $t$ \textit{conditioned} on not having collided before time $t$ will often be close to~1.
%As an intuitive example of this, consider a human who can choose to traverse one of two narrow passages: as the robot plans a trajectory through the left passage, the probability of colliding with the human becomes smaller over time as we condition on no collisions having occurred so far, because there is increasing evidence that the human chose the right passage, and therefore no collisions will take place.}
%We therefore opt for a different approximation: rather than providing a highly conservative upper bound for the probability of collision throughout a robot trajectory,
Since assuming independence of collision probabilities over time is both unrealistic and overly conservative, we instead seek to find a tight lower bound on a trajectory's overall collision probability based on the marginal probabilities at each moment in time. In particular, based on the positive correlation
over time resulting from human motion continuity,
we first consider replacing each conditional probability
$P\big(x_H^\tau\not\in \mathcal{H}_\mathcal{E}(x_R^\tau)
    \mid x_H^s\not\in \mathcal{H}_\mathcal{E}(x_R^s), t\le s<\tau\big)$
    by $1$ for all $t>0$.
This would then give the lower bound
\begin{equation}\label{eq:lower_bound}
    P^{t:T}_\text{coll}\ge 1-P\big(x_H^t\not\in \mathcal{H}_\mathcal{E}(x_R^t)\big)
    = P\big(x_H^t\in \mathcal{H}_\mathcal{E}(x_R^t)\big)
    \enspace ,
\end{equation}
which would seem like an unreasonably optimistic approximation.
However, note that probabilities can be conditioned in any particular order (not necessarily chronological) and we can therefore generate $T-t+1$ lower bounds of the form $P^{t:T}_\text{coll}\ge P\big(x_H^\tau\in \mathcal{H}_\mathcal{E}(x_R^\tau)\big)$ 
for $\tau\in\{t,\hdots,T\}$, again by replacing all successive conditional non-collision probabilities by~1.
Taking the tightest of all of these bounds, we can obtain an informative, yet quickly computable, approximator for the sought probability:
\begin{equation}\label{eq:prob_approx}
    P^{t:T}_\text{coll} \approx \max_{\tau\in\{t:T\}}P\big(x_H^{\tau}\in \mathcal{H}_\mathcal{E}(x_R^{\tau})\big)
    \enspace .
\end{equation}
In other words, we are replacing the probability of collision of an entire trajectory with the highest marginal collision probability at \textit{each point} in the trajectory.
While this approximation will err on the side of optimism, we note that the robot's ability to continually replan as updated human predictions become available mitigates any potentially underestimated risks, since in reality the robot does not need to commit to a plan that was initially deemed safe, and will readily rectify as the estimated collision risk increases prior to an actual collision.

\example{
%The keep-out set~$\mathcal{K}$ and the tracking error bound~$\mathcal{E}$ are boxes of dimension 5 and 3 respectively.
Given $\mathcal{K}$ and $\mathcal{E}$,
$\mathcal{H}_\mathcal{E}(x_R^\tau)$ is the set of human positions within the rectangle of dimensions ${(l+\mathcal{E}_x) \times (l+\mathcal{E}_y)}$ centered on $[p_x^\tau,p_y^\tau]$.
A human anywhere in this rectangle could be in collision with the quadcopter.
}

\subsection{Safe Online Planning under Uncertain Human Predictions}

We can now use this real-time evaluation of collision probabilities to discriminate between valid and invalid trajectory candidates in the robot's online motion planning.
Using the formulation in Section~\ref{sec:solution_pred}, we can quickly generate, at every time~$t$, the marginal probabilities in \eqref{eq:prob_approx} at each future time $\tau \in\{t,\hdots,T\}$, based on past observations at times $0,\hdots,t$.
Specifically, for any candidate trajectory point $x_R^\tau$, we first calculate the set $\mathcal{H}_\mathcal{E}(x_R^\tau)$;
this set can often be obtained analytically from \eqref{eq:H_E}, and can otherwise be numerically approximated from a discretization of $\mathcal{E}$.
The planner then computes the instantaneous probability of collision $P\big(x_H^\tau\in \mathcal{H}_\mathcal{E}(x_R^\tau)\big)$ by integrating $P\big(x_H^{\tau} \mid x_H^{0:t}\big)$ over $\mathcal{H}_\mathcal{E}(x_R^\tau)$, and rejects the candidate point $x_R^\tau$ if this probability exceeds $P_{\text{th}}$.

Note that for search-based planners that consider candidate trajectories by generating a tree of timestamped states, rejecting a candidate node from this tree is equivalent to rejecting all further trajectories that would contain the node. This early rejection rule is consistent with the proposed approximation \eqref{eq:prob_approx} of $P^{t:T}_\text{coll}$ while preventing unnecessary exploration of candidate trajecories that would ultimately be deemed unsafe.



% \jfnote{What follows is an old version for what we really propose doing, which is approximate the joint by the max}.
% In particular, for every pair $(t, x_R^t)$ explored by the planner, we compute the probability mass from the human's predicted occupancy distribution enclosed within the tracking error bound around $x_R^t$. \abnote{Add in figure or flowchart of how the whole system works together.}
% Since FaSTrack's guarantee states that, at worst, the robot could find itself anywhere within this bound at time $t$ while attempting to follow the candidate motion plan, this probability mass is equal to the probability that the human and the robot will be in collision under the worst-case robot tracking.
% \jfnote{Argue that $P(\text{crash}_{0:T}) \approx\max_t P(\text{crash}_t)$. }

As the robot is continuously regenerating its motion plan online as the human's predicted motion is updated, we simultaneously track the planned trajectory using our error feedback controller, which ensures that we deviate by no more than the tracking error bound $\mathcal{E}$. This planning and tracking procedure continues until the robot's goal has been achieved.
\\ \indent
\begin{figure}
\includegraphics[width=.48\textwidth]{coffee_three_quadrotor.pdf} 
\caption{Scenario from Fig. \ref{fig:coffee_six} visualized with robot's trajectory based on its current $\beta$. When $\beta$ is low and the robot is not confident, it makes large deviations from its path to accommodate the human. When $\beta$ is high, the robot refuses to change course and comes dangerously close to the human. With inferred model confidence, the robot balances safety and efficiency with a slight deviation around the human.}
\label{fig:coffee_three_quadrotor}
\vspace{-0.7cm}
\end{figure}
\example{
    Our quadcopter is now required to navigate to a target position shown in Fig. \ref{fig:coffee_six} without colliding with the human. Our proposed algorithm successfully avoids collisions at all times, replanning to leave greater separation from the human whenever her motion departs from the model. In contrast, robot planning with fixed model confidence is either overly conservative at the expense of time and performance or overly aggressive at the expense of safety.
    %\jfnote{Parallel path: $\beta$-estimating quadrotor deviates iff human is being ``noisy")}.
}

% \begin{figure}[h]
% \centering
% \includegraphics[width=.4\textwidth]{figs/triangle_quadrotor.pdf} 
% \caption{This example shows the same captured human data from Fig. \ref{fig:triangle_three} with added quadcopter trajectories. For clarity we show the trajectories over two sets in time, with the human navigating to the first known goal on the left, and the human navigating to the second known goal and back to the start on the right. The quadcopter wants to move across the scene and back again. Note that by the inferred model confidence, the robot safely avoids the human while maintaining a fairly direct route to its goal.\adnote{this figure is a little tricky to parse -- not sure if there are collisions or not, not sure what's wrong with low confidence (seems like on the first part when confidence should be high , beta low confidence produces the same path pretty much? and then when confidence should be low, beta low confidence produces a different path but it's actually correct in its low confidence prediction and should do the same as beta inference}}
% \label{fig:triangle_quadrotor}
% \end{figure}
% Old stuff below
%
%
% Let $\tstate$ and $\tctrl$ be the robot's state and controls in the higher-fidelity \textit{tracking model}. The robot's dynamics evolve via the ordinary differential equation:
% \begin{equation}
%     \label{eq:tdyn}
%     \dot{\tstate} = \tdyn(\tstate, \tctrl, \dstb)
%     \enspace .
%     % \tvar \in [0, \thor]
% \end{equation}
%  The proposed approach applies to any time-varying planner, as long as its output can be interpreted as a trajectory of the planning model, given by: 
% \begin{equation}
%     \label{eq:pdyn}
%     \dot{\pstate} = \pdyn(\pstate, \pctrl)
%     \enspace .
%     % \tvar \in [0, \thor]
% \end{equation}
    % In this paper we use space-time A*.
    %\item We want to track the planner with our dynamic robot while maintaining safety.
 %To generate tracking error bound and corresponding error feedback controller, FaSTrack analyses a differential game based on relative dynamics between the tracking and planning models. This analysis results in the maximum distance possible between two systems (i.e. the tracking error bound), along with a error feedback controller (implemented as a look-up table) that takes in the current relative state and outputs the optimal control for the robot to track the planner.
 %Online, we can plan using a time-varying motion planner (in particular, we implement space-time A*).
